Learning Solution Manifolds for Control Problems via Energy Minimization

A variety of control tasks such as inverse kinematics (IK), trajectory optimization (TO), and model predictive control (MPC) are commonly formulated as energy minimization problems. Numerical solutions to such problems are well-established. However, these are often too slow to be used directly in real-time applications. The alternative is to learn solution manifolds for control problems in an offline stage. Although this distillation process can be trivially formulated as a behavioral cloning (BC) problem in an imitation learning setting, our experiments highlight a number of significant shortcomings arising due to incompatible local minima, interpolation artifacts, and insufficient coverage of the state space. In this paper, we propose an alternative to BC that is efficient and numerically robust. We formulate the learning of solution manifolds as a minimization of the energy terms of a control objective integrated over the space of problems of interest. We minimize this energy integral with a novel method that combines Monte Carlo-inspired adaptive sampling strategies with the derivatives used to solve individual instances of the control task. We evaluate the performance of our formulation on a series of robotic control problems of increasing complexity, and we highlight its benefits through comparisons against traditional methods such as behavioral cloning and Dataset aggregation (Dagger).

==> chapters/20_preliminaries.tex <==
\section{Preliminaries}

% Outline:

% \begin{itemize}
%     \item Introduce energy minimization in Trajectory Space (TS) a.k.a  Trajectery optimization (TO) (1st and 2nd order)
%     \item Introduce energy minimization in Parameter Space (PS) (1st and 2nd order)
%     \item Casting 1st order energy minimization in PS to 1st order supervised learning.
%     \begin{itemize}
%         \item Introduce target trick to match update rules in PS.
%         \item Make relation to energy minimization in TS (Learning intermediate solutions of TO)
%         \item Explain effect of line search in parameter space.
%     \end{itemize}
    
%     \item Casting 2nd order energy minimization in PS to 2nd order supervised learning.
%     \begin{itemize}
%         \item Show how casting the problems motivates the introduction of the weighting matrix M 
%         \item Make relation to energy minimization in TS (Learning intermediate solutions of TO)
%         \item Explain effect of line search in parameter space.
%         \item Explain limitations of setting M for each data point in batch mode.
%     \end{itemize}
    
%     \item Trade-offs and simplifications
%     \begin{itemize}
%         \item Energy minimization in TS with Gauss-Newton. (Ensures invertibility)
%         \item 2nd order methods in PS expensive but 2nd order info from TS is tractable and helpful. how to incorporate 2nd order info from TS?
%         \item 1st order supervised learning with 1st target and special weighting matrix M. (Incorporates second order info in TS but still batch mode problem )
%         \item Equivalent result obtained with 1st order supervised learning and Gauss-Newston target. (Removes batch problem of weighting Matrix)
%         \item Compare update rule against 2nd order supervised learning with second order target. (Neglecting third order tensors and network jacobian these can be equivalent)
%     \end{itemize}
    
% \end{itemize}

\subsection{Energy minimization in trajectory space}\label{section:e_min_TS}
- {\color{blue} Note on convention: }
In the following derivations we assume vectors are column vectors and we use a numerator layout for the derivatives, that is the derivative of a scalar function w.r.t to a vector is a row vector. \newline 

For an initial state $\sVec_0$, a state trajectory $\sVec := [\sVec_1^T, \dots, \sVec_{t}^T]^T$, and a control trajectory $\aVec := [\aVec_0^T, \dots, \aVec_{t-1}^T]^T$, we define an Energy function
\begin{alignat}{4}
    &  E  \,\, &  = & \,\,  E( \sVec(\aVec, \sVec_0), \aVec, \sVec_0)  \nonumber
\end{alignat}  

Where $\sVec(\aVec, \sVec_0)$ denotes the fact that the trajectory of states depends on the trajectory of actions and the initial conditions, and our goal is then to minimize such energy over the set of initial conditions of interest $S$,  that is:

\begin{alignat}{4}
&   &   & \,\,  min  \int _{ S }^{  }{ E( \sVec(\aVec, \sVec_0), \aVec, \sVec_0) \,\, d\sVec_{0}}   \nonumber
\end{alignat}  

To minimize the energy associated to a single initial condition $\sVec_0$ we can rely on TO methods. For a differentiable energy function and following the formulation presented in  \cite{puppetMaster}, we can derive an iterative optimization procedure that updates the control trajectory using one of the following update rules:

- First order update rule
\begin{alignat}{4}
    &  \aVec  \,\, & \xleftarrow{}  & \,\, \aVec - \alpha_{\aVec} \biggl[ \dv{ E( \sVec(\aVec), \aVec ) }{\aVec} \biggr]^{T}  \label{eq:TS_1st_update}
\end{alignat}

- Second order update rule
\begin{alignat}{4} 
    &  \aVec  \,\, & \xleftarrow{}  & \,\, \aVec - \alpha_{\aVec} {\biggl[ \dv[2]{E( \sVec(\aVec), \aVec )}{\aVec}  \biggr]}^{-1} \biggl[ \dv{ E( \sVec(\aVec), \aVec ) }{\aVec}  \biggr]^{T} \label{eq:TS_2nd_update}
\end{alignat}

where we dropped the dependency on $\sVec_0$ for simplicity of notation, $\dv{ E( \sVec(\aVec), \aVec ) }{\aVec}$ is the gradient, $\dv[2]{E( \sVec(\aVec), \aVec )}{\aVec}$ is the hessian of the energy function w.r.t the control trajectory, and $\alpha_{\aVec}$ is a learning rate that is set dynamically using a line search procedure. Furthermore, the hessian in the second order update rule can be replaced by its Gauss-Newton approximation that is guaranteed to be positive definite.  

Algorithm \ref{alg:EM_TS} summarizes the overall approach for energy minimization in TS.


\begin{algorithm}%[tb]
   \caption{Energy Minimization in TS}
   \label{alg:EM_TS}
\begin{algorithmic}
   \STATE {\bfseries Input:} $\sVec_0, \aVec_0$
   \FOR{$k=1$ {\bfseries to} $K$}
   \STATE // Recall $\sVec \coloneqq \sVec(\aVec, \sVec_0 )  $
   \STATE $\aVec_{k}   \xleftarrow{}  \aVec_{k-1} - \alpha_{\aVec} \biggl[ \dv{ E( \sVec, \aVec_{k-1}, \sVec_0 )  }{\aVec_{k-1}} \biggr]^{T} $ or using eq. \ref{eq:TS_2nd_update}
   \ENDFOR
\end{algorithmic}
\end{algorithm}


\textbf{- Behavioral Cloning using energy minimization in TS:}
\begin{itemize}
    \item Considering the IK problem of a 2-Link mechanism, we can use energy minimization in TS to build a dataset  for behavioral cloning.
    \item Such simple problem allows to sample densely and investigate the overall energy landscape associated with a policy obtained via BC on a sparse training set (Figure \ref{fig:BC_energy_2Link}).  (ie allows us to examine generalization capabilities)
    \item Both circle and triangle markers denote samples of the input space for which we used energy minimization in TS to find an IK solution. 
    \item A closer look at the regions were the BC policy performs poorly (red) reveals the problem of conflicting data.
    
    \item At every point in the reachable workspace space of the 2-link mechanism there exist two solutions, namely the elbow-up and elbow-down solutions. Now consider a small dataset of two points $s_1$, $s_2$, where the former has an elbow up solution and the later has an elbow down solution (Figure \ref{fig:Conflicting_data}). If we interpolate the solutions associated to points $s_1$ and $s_1$, we get a possible solution for point $s_3$ (Which is exactly what happens when minimizing and L2-norm, \MZ{Highlight this better? Recalling that training neural nets by minimizing an L2 norm is equivalent to solving a least squares problem, which leads to an interpolation effect for the points of state space that are not part of the training set. }).
\end{itemize}


\subsection{Energy minimization in parameter space}
Control trajectories can also be generated using a neural network $\piPVec$ parametrized by $\thetaVec$ that produces a one shot trajectory of actions given an initial state  $\piPVec(\sVec_0) := [\aVec_0^T, \dots, \aVec_{t-1}^T]^T$.  The energy integral can then be defined as follows:
\begin{alignat}{4}
&   &   & \,\,  min  \int _{ S }^{  }{ E( \sVec(\piPVec, \sVec_0), \piPVec, \sVec_0 )  \,\, d\sVec_{0}}   \nonumber
\end{alignat} 

Where $\sVec(\piPVec, \sVec_0)$ denotes the fact that the trajectory of states depends on the initial state $\sVec_0$ and on the trajectory of actions generated by the $\piPVec$. As in the case of TO we can define first and second order update rules in terms of the gradient and the hessian of the energy w.r.t the parameters $\thetaVec$. For simplicity of notation we drop again the dependency on $\sVec_0$:

- First order update rule
\begin{alignat}{4}
    &  \thetaVec  \,\, & \xleftarrow{}  & \,\, \thetaVec - \alpha_{\thetaVec} \biggl[ \dv{ E( \sVec(\piPVec), \piPVec ) }{\thetaVec}  \biggr]^{T}  \label{eq:PS_1st_update}
\end{alignat}

- Second order update rule
\begin{alignat}{4}
    &  \thetaVec  \,\, & \xleftarrow{}  & \,\, \thetaVec - \alpha_{\thetaVec} {\biggl[ \dv[2]{E( \sVec(\piPVec), \piPVec )}{\thetaVec}  \biggr]}^{-1} \biggl[ \dv{ E( \sVec(\piPVec), \piPVec ) }{\thetaVec}  \biggr]^{T} \label{eq:PS_2nd_update}
\end{alignat}

Note however that evaluating the previous update rules requires evaluating the same type of gradients and hessians that are use for TO plus additional gradients and hessians of $\piPVec$ w.r.t $\thetaVec$. Applying the chain rule to the gradient $\dv{ E( \sVec(\piPVec), \piPVec ) }{\thetaVec}$, for example,  we get:

\begin{alignat}{4}
    &  \dv{ E( \sVec(\piPVec), \piPVec ) }{\thetaVec}  \,\, & =  & \,\, \dv{ E( \sVec(\piPVec), \piPVec ) }{\piPVec} \dv{ \piPVec }{\thetaVec} \nonumber
\end{alignat}

where the term $\dv{ E( \sVec(\piPVec), \piPVec ) }{\piPVec}$ is the gradient of the energy function w.r.t the actions that $\piPVec$ outputs i.e it is exactly equivalent to $\dv{ E( \sVec(\aVec), \aVec ) }{\aVec}$. The full expression for hessian $\dv[2]{E( \sVec(\piPVec), \piPVec )}{\thetaVec}$ is presented in the appendix \ref{appdx:full-hessian-theta}.

Algorithm \ref{alg:EM_PS} summarizes the overall approach for energy minimization in PS.

\begin{algorithm}%[tb]
   \caption{Energy Minimization in PS}
   \label{alg:EM_PS}
\begin{algorithmic}
   \STATE {\bfseries Input:} $\sVec_0$
   \FOR{$n=1$ {\bfseries to} $N$}
   \STATE // Recall $ \piPVec \coloneqq \piPVec(\sVec_0) $
   \STATE // Recall $ \sVec \coloneqq \sVec( \piPVec, \sVec_0) $
   
   \STATE $\thetaVec_{n}   \xleftarrow{}  \thetaVec_{n-1} - \alpha_{\thetaVec} \biggl[ \dv{ E( \sVec, \piPVec[n-1], \sVec_0 ) }{\thetaVec_{n-1}}  \biggr]^{T} $  or using eq. \ref{eq:PS_2nd_update}
   \ENDFOR
\end{algorithmic}
\end{algorithm}



==> chapters/21_method.tex <==
\section{Method}
\subsection{Casting energy minimization as supervised learning}
While it is possible to embed the computation of all the gradients and hessian into an autodifferentiation framework to minimize the energy in parameter space, it is worth pointing out that over the years TO algorithms have specialized in computing derivatives of objective functions w.r.t  actions, while many deep learning frameworks have specialized in computing derivatives of neural networks w.r.t. their parameters. In an attempt to leverage the best of both worlds, we seek to feed TO information to a supervised learning framework in such a way as to obtain the same overall update rules as the ones required to minimize the energy in parameters space.

Let us then consider a supervised learning loss $L$ with a symmetric weighting matrix $W$ to be defined as follows:
\begin{alignat}{4}
    &  L  \,\, &  = & \,\, \frac{1}{2}(\piPVec(\sVec_0) - \TVec)^{T} W (\piPVec(\sVec_0) - \TVec) \nonumber \\
    &     \,\, &  = & \,\, \frac{1}{2} {|| \piPVec(\sVec_0) - \TVec||}_{W}^2  \nonumber
\end{alignat}    

As before, we can define update rules for such loss function:

- First order update rule:
\begin{alignat}{4}
    &  \thetaVec  \,\, & \xleftarrow{}  & \,\, \thetaVec - \alpha_{L} \biggl[ \dv{ L }{\thetaVec}  \biggr]^{T} \nonumber
\end{alignat}

- Second order update rule:
\begin{alignat}{4}
    &  \thetaVec  \,\, & \xleftarrow{}  & \,\, \thetaVec - \alpha_{L} {\biggl[ \dv[2]{ L }{\thetaVec} \biggr]}^{-1} \biggl[  \dv{ L }{\thetaVec} \biggr]^{T} \nonumber
\end{alignat}

where the gradient and hessian are defined as follows: 
\begin{alignat}{4}
    & \dv{ L }{\thetaVec}   \,\, & = & \,\, (\piPVec(\sVec_0) - \TVec)^{T} W \dv{ \piPVec }{\thetaVec} \nonumber \\
%    &                       \,\, &   & \nonumber \\
    & \dv[2]{ L }{\thetaVec} \,\, & = & \,\, \dv{ \piPVec }{\thetaVec}^{T}  W \dv{ \piPVec }{\thetaVec} +  
                        (\piPVec(\sVec_0) - \TVec)^{T  } W \dv[2]{ \piPVec }{\thetaVec}  \nonumber                  
\end{alignat}

Note that the target $\TVec$ and the matrix $W$ are two different mechanisms to feed information into the supervised update rules. \newline

%--------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------

\textbf{- First order supervised updates with first order targets:} \newline
Let us define a first order target, i.e a target that contains only first order information, as follows:
\begin{alignat}{4}
    &  \TVec  \,\, & = & \,\, \piPVec(\sVec_0) - \alpha_{\aVec} \dv{ E( \sVec(\piPVec), \piPVec ) }{\piPVec}^{T}\nonumber 
\end{alignat}

Feeding such target into the 1st order supervised update rule yields to:

\begin{alignat}{4}
    &  \thetaVec  \,\, & \xleftarrow{}  & \,\, \thetaVec - \alpha_{L} \alpha_{\aVec} \biggl[ \dv{ E( \sVec(\piPVec), \piPVec ) }{\piPVec} W \dv{ \piPVec }{\thetaVec}  \biggr]^{T} \nonumber
\end{alignat}

which matches the first order update rule for energy minimization by setting $W$ to the identity matrix and $\alpha_{L}$ accordingly. \newline

%--------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------

\textbf{- First order updates with second order targets:} 

Recalling first order update rule for energy minimization:
\begin{alignat}{4}
    &  \thetaVec  \,\, & \xleftarrow{}  & \,\, \thetaVec - \alpha_{\thetaVec} \biggl[ \dv{ E( \sVec(\piPVec), \piPVec ) }{\piPVec} \dv{ \piPVec }{\thetaVec}   \biggr]^{T} \nonumber
\end{alignat}
and first order update rule for supervised learning:
\begin{alignat}{4}
    &  \thetaVec  \,\, & \xleftarrow{}  & \,\, \thetaVec -\alpha_{L}\biggl[ (\piPVec(\sVec_0) - \TVec)^{T} W \dv{ \piPVec }{\thetaVec}  \biggr]^{T} \nonumber
\end{alignat}
defining a second order target:
\begin{alignat}{4}
    &  \TVec  \,\,  & = & \,\, \piPVec(\sVec_0) - \alpha_{\aVec} { \Hess }^{-1} \dv{ E( \sVec(\piPVec), \piPVec ) }{\piPVec}^{T}\nonumber 
\end{alignat}
where the Hessian $\Hess =\dv[2]{ E( \sVec(\piPVec), \piPVec ) }{\piPVec} $ is equivalent to the Hessian of Energy w.r.t to the control trajectory  $\bigl(\dv[2]{E( \sVec(\aVec, \sVec_0), \aVec ))}{\aVec}\bigr)$ that is used for Energy minimization in trajectory space, yields to an overall update rule for supervised learning:
\begin{alignat}{4}
    &  \thetaVec  \,\, & \xleftarrow{}  & \,\, \thetaVec - \alpha_{L} \alpha_{\aVec} \biggl[ \dv{ E( \sVec(\piPVec), \piPVec ) }{\piPVec}  { \Hess }^{-1}  W \dv{ \piPVec }{\thetaVec} \biggr]^{T} \nonumber
\end{alignat}
Setting $W$ to and identity results in the \textbf{Curry}  update rule.
\begin{alignat}{4}
    &  \thetaVec  \,\, & \xleftarrow{}  & \,\, \thetaVec - \alpha_{L}\alpha_{\aVec} \biggl[ \dv{ E( \sVec(\piPVec), \piPVec ) }{\piPVec}  { \Hess }^{-1}  \dv{ \piPVec }{\thetaVec}  \biggr]^{T} \nonumber
\end{alignat}

%--------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------

\textbf{- Weighted first order updates with first order targets:} 

Notice that the same result can be obtained by using a first order target and setting the weighting matrix $W =  \Hess^{-1}$

First order target:
\begin{alignat}{4}
    &  \TVec  \,\,  & = & \,\, \piPVec(\sVec_0) - \alpha_{\aVec}\dv{ E( \sVec(\piPVec), \piPVec ) }{\piPVec}^{T}\nonumber 
\end{alignat}
First order update rule for supervised learning:
\begin{alignat}{4}
    &  \thetaVec  \,\, & \xleftarrow{}  & \,\, \thetaVec - \alpha_{L} \biggl[ (\piPVec(\sVec_0) - T)^{T} W \dv{ \piPVec }{\thetaVec} \biggr]^{T}   \nonumber \\
    &             \,\, & \xleftarrow{}  & \,\, \thetaVec - \alpha_{L} \alpha_{\aVec} \biggl[ \dv{ E( \sVec(\piPVec), \piPVec ) }{\piPVec} W \dv{ \piPVec }{\thetaVec} \biggr]^{T} \nonumber \\
    &             \,\, & \xleftarrow{}  & \,\, \thetaVec - \alpha_{L} \alpha_{\aVec} \biggl[ \dv{ E( \sVec(\piPVec), \piPVec ) }{\piPVec} \Hess^{-1} \dv{ \piPVec }{\thetaVec} \biggr]^{T} \nonumber
\end{alignat}

{\color{blue} In other words \textbf{Curry} can also be seen as minimizing a weighted squared error loss using first order updates with incremental/dynamic first order targets.}

\textbf{- Second order updates with second order targets:}\\
Update rules for second order updates with second order targets are presented in the Appendix \ref{appdx:Full_2ndOrder}, however due to the computational cost of computing the Hessian of the output of the Neural Network policy w.r.t its parameters $\dv[2]{ \piPVec }{\thetaVec}$ such update rule is not consider in this work.

\begin{algorithm}%[tb]
   \caption{Energy Minimization with Curry}
   \label{alg:EM_Curry}
\begin{algorithmic}
   \STATE {\bfseries Input:} $\sVec_0$
   \FOR{$k=1$ {\bfseries to} $K$}
   \STATE $\aVec_{k-1}   \xleftarrow{}  \piPVec(\sVec_0)$
   \STATE // Improvement in TS
   \STATE $\aVec_{k}   \xleftarrow{}  \aVec_{k-1} - \alpha_{\aVec} \biggl[ \dv{ E( \sVec, \aVec_{k-1}, \sVec_0 )  }{\aVec_{k-1}} \biggr]^{T} $ or using eq. \ref{eq:TS_2nd_update}
   \FOR{$n=1$ {\bfseries to} $N$}
   \STATE // Improvement in PS
   \STATE $\thetaVec_{n}   \xleftarrow{}  \thetaVec_{n-1} - \alpha_{L} \biggl[ \dv{ L }{\thetaVec_{n-1}}
   \biggr\vert_{\TVec = \aVec_{k}} \biggr]^{T} $
   \ENDFOR
   \ENDFOR
\end{algorithmic}
\end{algorithm}

\textbf{- Notes:} \MZ{Find better name for this}
\begin{itemize}
    \item Algorithm \ref{alg:EM_Curry} summarizes the Curry approach for energy minimization. Note that when $N = 1$ and Eq \ref{eq:TS_1st_update} is used to update $\aVec_{k}$, Curry is equivalent to Energy Minimization in PS (Algorithm \ref{alg:EM_PS}). 
    
    \item In practice Curry uses $N > 1$, with second order targets (updating $\aVec_{k}$ with eq \ref{eq:TS_2nd_update}), which can be seen as doing Behavioral Cloning on the intermediate control trajectories  $\aVec_{k}$ of the energy minimization in TS (Algorithm \ref{alg:EM_TS}).
    
    \item Note that in practice Curry is minimizing the energy concurrently for a batch of initial states.
    
    \item Notice that Algorithm \ref{alg:EM_TS} requires an initial guess $\aVec_0$, while Algorithm \ref{alg:EM_Curry} sets the output of $\piPVec$ as an initial guess for the improvement in TS. It also means that if the initial output of the neural net is very poor, the improvement step can get stuck.  To avoid such problem, curry evaluates the energy of a default initial guess and also the energy of the improved control trajectory obtained from the network output. If the the energy of the improved control trajectory is larger than the energy of the default initial guess, the default initialization is used as target to minimize $L$.
    
    \item Using the same states space samples that were used for BC in Figure \ref{fig:BC_energy_2Link}, we trained Curry using the same computational resources that were employed to generate the training set for BC, and the same network initialization and we obtained a much better behaved energy landscape Figure \ref{fig:CurryLandscape}.
    
    
\end{itemize}


\subsection{Sources of conflicts}
\MZ{This section might not be necessary} \\
Taking the IK problem as an example we can see that:
\begin{itemize}
\item Interpolating $\pi$ vs $-\pi$ can lead to conflicts. However, this is solved by training the net to match $\sin{q}, \cos{q}$ instead of matching the angle $q$. 
\item Multiplicity of solutions and null space.
        \begin{itemize}
        \item Even when the null-space of a robot is zero, there exist multiple solutions to the IK problem, Elbow-up vs Elbow-down solutions, which can lead to high-energy regions.
        \item For robots where the null space is larger than zero there exist a manifold of solutions for the IK problem.
        \end{itemize}

\end{itemize}

However in a more general setting like a TO, we can consider the problem of going from point a to point b, while avoiding an obstacle. Two feasible solutions are avoiding the obstacle on the right or left site. However interpolating between those two solutions will lead to a catastrophic trajectory.


\subsection{Sampling and rejecting conflicting data}
Uniform sampling and Gaussian sampling are perhaps the most commonly used approaches to explore a state space in the context of policy learning. In this work we explore the use of Poisson-disk sampling (PDS) \cite{poisson_disk_sampling} to explore the state space \ref{fig:sampling}. A special feature of PDS is ensuring that two samples are not too close to each other. Such feature is useful to tackle conflicting data, as it facilitates implementing a rejection mechanism based on a variation of the traditional k-nearest neighbour,  namely the fixed-radius nearest neighbours.  


\begin{figure}
\centering
\begin{tikzpicture}%[framed]
\node[inner sep=0pt] (pend) at (0,0)    {\includegraphics[width = 0.95\columnwidth]{imgs/Sampling.pdf} }; %, cfbox=blue 1pt 1pt

%\node at (-7.6, 1.1) (handleTxt) [text width=1.0cm, align=center] { \footnotesize $a$};
%\node at (-7.8, 0.10) (massTxt) [text width=1.0cm, rotate=90, align=center] { \footnotesize $x$};
\end{tikzpicture} 
    \caption{Left: Uniform sampling. Right: Poisson-Disk sampling} 
    \label{fig:sampling}
\end{figure}

Recalling the insight presented in section \ref{section:e_min_TS}, that interpolating two conflicting data points and their corresponding labels leads to high energies, then we can encourage non-conflicting datasets by searching and removing the samples, that when interpolated with its nearest neighbours result in high energy. \MZ{This actually implies there is a lot of continuity or smoothness in the solution manifold? It might also require that samples are not too far apart.}

Algorithm \ref{alg:Reject} describes the rejection process that relies on a metric function $D$. Such metric function can be the energy itself. However for interpretability, it can also be any other function that describes discrepancy between two interpolated samples.  For the IK examples we used the position error as a metric, which allowed us to set the threshold $\epsilon$ in very intuitive way.


Note that for the Dataset, the solution $\aVec_m$ associated to $\sVec_m$ is not necessarily the final solution obtained after performing $K$ steps of Energy Minimization in TS, but in can also be an intermediate solution. In practice we apply this rejection mechanism to curry after every improvement step in TS and before performing and improvement step in PS.


\MZ{Perhaps rejecting all the samples associated to a conflict is a bit harsh but for now that's what it is.}

Figure \ref{fig:knn_sizes} shows how even with a relatively small number of samples, our rejection mechanism is able to detect regions with conflicting data. \MZ{In higher dims, data will be more sparse, can we say something about the scalability of KNN to higher dims, given that it seems to behave ok even with sparse samples in low dims?}.  

\begin{figure}%[h]
\centering
\begin{tikzpicture}%[framed]
\node[inner sep=0pt] (pend) at (0,0)    {\includegraphics[width = 0.95\columnwidth]{imgs/knn_different_size.png} }; %, cfbox=blue 1pt 1pt
\end{tikzpicture} 
    \caption{Detecting conflicts with different sizes for the testset \MZ{Better Img}} 
    \label{fig:knn_sizes}
\end{figure}



\begin{algorithm}[tb]
   \caption{Rejection Mechanism}
   \label{alg:Reject}
\begin{algorithmic}
   \STATE {\bfseries Input:} $Dataset = ( (\sVec_0, \aVec_0), \dots,  (\sVec_M, \aVec_M) ) $
   \FOR{$m=0$ {\bfseries to} $M$}
   \STATE Find neighbours of $\sVec_m$ within a radius of $r$
   \STATE Interpolate all neighbours to get $\sVec_{m_{avg}}$
   \STATE Interpolate associated solutions $\aVec_{m_{avg}}$
   \STATE Evalate and Store metric $D_m(\sVec_{m_{avg}}, \aVec_{m_{avg}})$
   \ENDFOR
   \STATE Compute average $D_{m_{avg}}$
   \FOR{$m=0$ {\bfseries to} $M$}
   \IF{ $D_{m} >  D_{m_{avg}} + \epsilon$ }
   \STATE Reject sample $m$ and all its neighbouring samples.
   \ENDIF
   \ENDFOR
\end{algorithmic}
\end{algorithm}




\subsection{Training approaches:}

\begin{itemize}
    \item  \textbf{Full batch supervised learning aka behavioural cloning}
    \begin{itemize}
        %\item [\textbf{- Full batch supervised learning aka behavioural cloning}]
        \item For this  approach we choose a set of initial states from region of interest using either uniform sampling or Poisson-disk-sampling.
        For each initial state we minimize the energy in trajectory space, using a second order optimizer and then we use full batch supervised learning on solutions generated by the optimizer.
        \item \MZ{ Why do you use full batch? } Either full batch or mini-batch will probably result in a conflicted energy landscape. \MZ{ Should we show an experiment? }
    \end{itemize}

    \item \textbf{Curry full batch}
    \begin{itemize}
        \item As before we choose a set of initial states, and for each iteration of \textbf{Curry},  we do a one-step-minimization of the energy using a first order o second order update rule, followed by behavioural cloning. The set of selected initial states is kept fixed for every iteration of \textbf{Curry}.
        \item \MZ{ Why not use mini-batch? } Same as full-batch SL.
    \end{itemize}
    
    \item \textbf{Curry MC}
    \begin{itemize}
        \item In contrast to \textbf{Curry}- Full-batch we change the set of initial states at every \textbf{Curry} iteration.
    \end{itemize}

    \item \textbf{Curry MC Dagger}
    \begin{itemize}
        \item We sample the region of state space of interest and we choose the sample with lowest energy as the initial sample for our training set.
        \item After every iteration we grow the training set adding new initial states sampling randomly from a Poisson distribution.
    \end{itemize}
    
    \item \textbf{Curry MC Metric Dagger}
    \begin{itemize}
        \item Same as \textbf{Curry MC Dagger}, however,  in contrast to a traditional Dagger approach, every time we update the training set by adding new samples we make sure to add samples that are close to the seeding sample, according to a given metric i.e. Euclidean norm, growing the dataset incrementally. \MZ{Should we add a picture to illustrate the growing process?}
    \end{itemize}
    
    \item \textbf{Curry MC Metric Dagger with rejection}
    \begin{itemize}
        \item Same as \textbf{Curry MC Metric Dagger}, but in addition we use a rejection mechanism on the growing training set to remove samples that can lead to conflicts in the landscape. See Algorithm \ref{alg:Reject}.
    \end{itemize}
\end{itemize}




==> chapters/50_discussion.tex <==
\section{Discussion}

For rebutall porposes.


